Tokenize the World into Object-level Knowledge to Address Long-tail Events in Autonomous Driving

The autonomous driving industry is increasingly adopting end-to-end learning from sensory inputs to minimize human biases in system design. Traditional end-to-end driving models, however, suffer from long-tail events due to rare or unseen inputs within their training distributions. To address this, we propose TOKEN, a novel Multi-Modal Large Language Model (MM-LLM) that tokenizes the world into object-level knowledge, enabling better utilization of LLM's reasoning capabilities to enhance autonomous vehicle planning in long-tail scenarios. TOKEN effectively alleviates data scarcity and inefficient tokenization by leveraging a traditional end-to-end driving model to produce condensed and semantically enriched representations of the scene, which are optimized for LLM planning compatibility through deliberate representation and reasoning alignment training stages. Our results demonstrate that TOKEN excels in grounding, reasoning, and planning capabilities, outperforming existing frameworks with a 27% reduction in trajectory L2 error and a 39% decrease in collision rates in long-tail scenarios. Additionally, our work highlights the importance of representation alignment and structured reasoning in sparking the common-sense reasoning capabilities of MM-LLMs for effective planning.

==> sections/agent_driver_token_compare_table_full.tex <==
\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|l|lllll|lllll|lllll|c}
\toprule
& & \multicolumn{5}{c|}{Traj L2 (m) $\downarrow$ } & \multicolumn{5}{c|}{Heading L2 (rad) $\downarrow$} & 
\multicolumn{5}{c|}{Lon. weighted traj L2 (m) $\downarrow$} &
\multicolumn{1}{c}{Collision (\%) $\downarrow$} \\ 
Split & Method &  1s & 2s  & 3s  & Ave$_{123\text{s}}$  & Ave$_\text{all}$  & 1s & 2s  & 3s  & Ave$_{123\text{s}}$  & Ave$_\text{all}$ & 1s & 2s  & 3s  & Ave$_{123\text{s}}$  & Ave$_\text{all}$ & Ave$_\text{all}$ \\ \midrule
val & \multicolumn{1}{l|}{\new{Agent-Driver}} &  \textbf{\new{0.23}} & \textbf{ \new{0.68}}   &  \new{1.50} &  \textbf{\new{0.80}} &  \textbf{\new{0.66}}  &  \new{0.79}  & 0.85 & 0.90 & 0.85 & 0.80 & \textbf{0.43} & \textbf{1.26} & 2.75 & \textbf{1.48} & \textbf{1.22} & \textbf{0.13}\\ 
& \multicolumn{1}{l|}{\token} & \new{0.26} & \new{0.70}   &  \textbf{\new{1.46}} &  \new{0.81} &\new{0.68}  &  \textbf{\new{0.13}}  &  \textbf{0.18} & \textbf{0.21} & \textbf{0.17} & \textbf{0.18} & 0.50 & 1.32 & \textbf{2.72} & 1.51 & 1.26 & 0.15\\
& \multicolumn{1}{l|}{\token$^+$} & \new{0.17} & \new{0.52}   &  \new{1.21} &  \new{0.64} &\new{0.52}  &  \new{0.10}  &  0.16 & 0.19 & 0.15 & 0.17 & 0.33 & 1.00 & 2.30 & 1.21 & 1.00 & 0.13\\ 
\midrule
 3-point turn & \multicolumn{1}{l|}{\new{Agent-Driver}} &  \textbf{\new{0.38}} &  \new{1.31}   &  \new{2.93} &  \new{1.54} &  \new{1.26}  &  \new{0.20}  & 0.74 & 1.23 & 0.72 & 0.63 & \textbf{0.64} & 2.26 & 4.78 & 2.56 & 2.11 & 8.67\\ 
& \multicolumn{1}{l|}{\token} & \new{0.39} &  \textbf{\new{1.29}}   &  \textbf{\new{2.60}} &  \textbf{\new{1.43}} &  \textbf{\new{1.18}}  &  \textbf{\new{0.21}}  & \textbf{0.35} & \textbf{0.71} & \textbf{0.42} &  \textbf{0.36} & 0.68 & \textbf{2.15} & \textbf{4.33} & \textbf{2.39} & \textbf{1.98 }& \textbf{4.00}\\
& \multicolumn{1}{l|}{\token$^+$} & \new{0.20} & \new{0.73}   &  \new{1.77} &  \new{0.90} &\new{0.73}  &  \new{0.17}  &  0.22 & 0.38 & 0.26 & 0.22 & 0.37 & 1.28 & 2.93 & 1.53 & 1.24 & 1.46\\ 
\midrule 

Resume motion & \multicolumn{1}{l|}{\new{Agent-Driver}} &  \new{0.14} &  \new{0.84}   &  \new{2.51} &  \new{1.16} &  \new{0.91}  &  \new{0.17}  & 0.47 & 0.42 & 0.35 & 0.32 & 0.25 & 1.49 & 4.48 & 2.07 & 1.62 & 0.00\\ 
from full stop & \multicolumn{1}{l|}{\token} & \textbf{\new{0.13}}   &  \textbf{\new{0.70}} &  \textbf{\new{1.58}} & \textbf{\new{0.80}}  &  \textbf{\new{0.65}}  & \textbf{0.09} & \textbf{0.24} & \textbf{0.31} & \textbf{0.22} & \textbf{0.19} & \textbf{0.24} & \textbf{1.24} & \textbf{2.66} & \textbf{1.38} & \textbf{1.13} & 0.00\\ 
%
& \multicolumn{1}{l|}{\token$^+$} & \new{0.06} & \new{0.43}   &  \new{1.27} &  \new{0.59} &\new{0.46}  &  \new{0.05}  &  0.13 & 0.17 & 0.12 & 0.10 & 0.11 & 0.78 & 2.30 & 1.06 & 0.84 & 0.00\\ 
\midrule 
%
Overtake & \multicolumn{1}{l|}{\new{Agent-Driver}} &  \textbf{\new{0.27}} &  \new{0.89}   &  \new{2.07} &  \new{1.08} &  \new{0.88}  &  \new{0.05}  & 0.13 & 0.24 & 0.14 & 0.12 & \textbf{0.47} & 1.46 & 3.37 & 1.77 & 1.45 & 0.77\\ 
& \multicolumn{1}{l|}{\token} &  \new{0.29}   &  \textbf{\new{0.77}} &  \textbf{\new{1.63}} & \textbf{\new{0.90}}  & \textbf{ \new{0.74}}  &  \textbf{0.04} &  \textbf{0.07} & \textbf{0.11} & \textbf{ 0.07} & \textbf{0.09} & 0.53 & \textbf{1.36} & \textbf{2.86} &  \textbf{1.58} &  \textbf{1.31} &  \textbf{0.19}\\
& \multicolumn{1}{l|}{\token$^+$} & \new{0.15} & \new{0.46}   &  \new{1.04} &  \new{0.55} &\new{0.46}  &  \new{0.02}  &  0.07 & 0.13 & 0.07 & 0.06 & 0.29 & 0.83 & 1.75 & 0.95 & 0.80 & 0.00\\
\midrule 
% Yield & \multicolumn{1}{l|}{\new{Agent-Driver}} &  \textbf{\new{0.21}} &  \new{0.77}   &  \new{1.78} &  \new{0.92} &  \new{0.75}  &  \new{1.08}  & 1.40 & 1.88 & 1.46 & 1.29 & \textbf{0.40} & 1.51 & 3.50 & 1.80 & 1.47 & 0.32\\ 
% & \multicolumn{1}{l|}{\token} & \textbf{\new{0.22}}   &   \textbf{\new{0.71}} &   \textbf{\new{1.49}} &  \textbf{\new{0.81}}  &   \textbf{\new{0.67}}  &  \textbf{0.15} &  \textbf{0.30} &  \textbf{0.49} &  \textbf{0.31} &  \textbf{0.29} & 0.44 &  \textbf{1.41} &  \textbf{2.95} &  \textbf{1.60} &  \textbf{1.33} &   \textbf{0.00}\\
% & \multicolumn{1}{l|}{\token$^+$} & \new{0.11} & \new{0.40}   &  \new{1.06} &  \new{0.52} &\new{0.42}  &  \new{0.13}  &  0.30 & 0.48 & 0.30 & 0.25 & 0.20 & 0.78 & 2.07 & 1.02 & 0.83 & 0.00\\
%\midrule 
\end{tabular}
}
\caption{\textbf{Quantitative comparison with an LLM-based planner - Agent-Driver.} \token significantly outperforms Agent-Driver in long-tail scenarios. TOKEN$^+$ denotes a variant of TOKEN that uses ego-state as input, similar to Agent-Driver.}
\label{tab: token_vs_Agent-Driver_ood_full} 
\end{table*}
